Evolving simple programs for playing Atari games

Cartesian Genetic Programming (CGP) has previously shown capabilities in image processing tasks by evolving programs with a function set specialized for computer vision. A similar approach can be applied to Atari playing. Programs are evolved using mixed type CGP with a function set suited for matrix operations, including image processing, but allowing for controller behavior to emerge. While the programs are relatively small, many controllers are competitive with state of the art methods for the Atari benchmark set and require less training time. By evaluating the programs of the best evolved individuals, simple but effective strategies can be found.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios
		Code prettying (Michael D. Adams)
		Two-column formats now balance the last page (ACM request)
		

==> grn.tex <==
\section{Genetic Regulatory Networks}
\label{sec:grn}

The GRN described in this section was designed by Banzhaf in
\cite{banzhaf2003artificial}, with modifications made in \cite{Chavoya2008}. The
components under review in this study are further explored in
\autoref{sec:dynamics}.

A GRN is composed of multiple artificial proteins, which interact via evolved
properties. These properties, called tags, are
\begin{itemize}

\item The protein \emph{identifier}, encoded as an integer between 0 and
  $u_{size}$. $u_{size}$ can be changed in order to control the precision of the
  GRN.

\item The \emph{enhancer identifier}, encoded as an integer between 0 and $u_{size}$.
  The enhancer identifier is used to calculate the enhancing matching factor
  between two proteins.

\item The \emph{inhibitor identifier}, encoded as an integer between 0 and $u_{size}$.
  The inhibitor identifier is used to calculate the inhibiting matching factor
  between two proteins.

\item The \emph{type}, either \emph{input}, \emph{output}, or \emph{regulator}. The type is a constant set by the user and is not evolved.

\end{itemize}

Each protein has a concentration, representing the use of this protein and
proving state to the network similar to neurotransmitter concentrations in
spiking neural networks (SNN). For \emph{input} proteins, the concentration is given
by the environment and is unaffected by other proteins. \emph{output} protein
concentrations are used to determine actions in the environment; these proteins
do not affect others in the network. The bulk of the computation is performed by
\emph{regulatory} proteins, an internal protein whose concentration is
influenced by other \emph{input} and \emph{regulatory} proteins.

The dynamics of the GRN are calculated as follows. First, the absolute affinity of a
protein $a$ with another protein $b$ is given by the enhancing factor
$u^{+}_{ab}$ and the inhibiting $u^{-}_{ab}$:
\begin{equation}
\label{eq:affinity_first}
u^{+}_{ij}=u_{size}-|enh_j-id_i|~~;~~u^{-}_{ij}=u_{size}-|inh_j-id_i|
\end{equation}

where $id_x$ is the identifier, $enh_x$ is the enhancer identifier and $inh_x$
is the inhibitor identifier of protein $x$. The maximum enhancing and inhibiting
affinities between all protein pairs are determined and are used to calculate the relative affinity, which is here simply called the affinity:
\begin{equation}
\label{eq:affinity_main}
A^{+}_{ij}=\beta(u^{+}_{ij}-u_{max}^{+})~~;~~A^{-}_{ij}=\beta(u^{-}_{ij}-u_{max}^{-})
\end{equation}
$\beta$ is one of two control parameters used in a GRN, both of which are
described below. Variants of this equation used in this study are detailed in
\autoref{sec:affinity}.

These affinities are used to then calculate the enhancing and inhibiting
influence of each protein, following
\begin{equation}
\label{eq:dynamics_1}
g_i=\frac{1}{N}\sum_j^N{c_je^{A^{+}_{ij}}}~~;~~h_i=\frac{1}{N}\sum_j^N{c_je^{A^{-}_{ij}}}
\end{equation}
where $g_i$ (resp. $h_i$) is the enhancing (resp. inhibiting) value for a
protein $i$, $N$ is the number of proteins in the network, $c_j$ is the
concentration of protein $j$. The use of an exponential in this function, as
opposed to other operations, is examined in \autoref{sec:inf_func}

The final modification of protein $i$ concentration is given by the following
differential equation:
\begin{equation}
\label{eq:dynamics_2}
\frac{dc_i}{dt}=\frac{\delta(g_i-h_i)}{\Phi}
\end{equation}
where $\Phi$ is a function that normalizes the output and regulatory protein
concentrations to sum to 1. The use of normalization is explored in
\autoref{sec:normalization}

$\beta$ and $\delta$ are two constants that determine the speed of reaction of
the regulatory network. The higher these values, the more sudden the transitions
in the GRN. The lower they are, the smoother the transitions. For this paper,
they are evolved as part of the GRN chromosome and are both kept within the
range $[0.5, 2.0]$.

\subsection{GRNEAT}
\label{sec:GRNEAT}

Gene Regulatory Network Evolution Through Augmenting Topologies (GRNEAT) is a
specialized Genetic Algorithm for GRN evolution proposed in
\cite{Cussat-Blanc2015a} and based on Stanley's NeuroEvolution of Augmenting
Topologies (NEAT) algorithm \cite{Stanley2002}. This algorithm has been shown to
improve evolution performance on neural networks, complex pattern producing
networks, and GRNs\cite{stanley2009hypercube}. A major contribution is the
design of a crossover method for network controllers, in which structure has a
significant influence on overall network behavior. GRNEAT uses a similar
crossover, and imports three key elements from NEAT:

\begin{itemize}
  \item the initialization of the algorithm - small networks are generated that
    resemble a select subpopulation termed initial species leaders
  \item speciation, which limits competition and crossover to similar
    individuals. This both protects some new mutants from immediately competing
    with champion individuals and protects novel solutions by allowing them to
    optimize their structures before competing with the whole population
 \item an alignment crossover that compares individual genes before selection
   for a new individual
\end{itemize}

The distance metric in this paper for speciation and alignment crossover was 
\begin{equation}
D_{prot}(i,j) = \frac{a|id_i-id_j|+b|enh_i-enh_j|+c|inh_i-inh_j|}{u_{size}}
\end{equation}
where $a=0.75$, $b=0.125$, and $c=0.125$. Proteins were aligned in each GRN
during comparison first based on \emph{type} and secondly based on minimum
$D_{prot}(A,B)$. The distance between GRNs was then calculated as
\begin{gather*}
D(G_1,G_2) = \frac{D_{in} + D_{out} + D_{reg} + D_{\beta} + D_{\delta}}{max(N_1,N_2)+2}\\
D_{\beta} = \frac{\beta_1 - \beta_2}{\beta_{max} - \beta_{min}}\\
D_{\delta} = \frac{\delta_1 - \delta_2}{\delta_{max} - \delta_{min}}
\end{gather*}
where $N_i$ is the number of proteins in GRN $G_i$, and $D_{\emph{type}}$ is the
sum of the difference of all aligned proteins of that \emph{type}. For
regulatory proteins, where $N$ can differ between two GRNs, the distance for all
non-aligned proteins was taken between the protein parameters and $u_{size}$.
The use of alignment without replacement for the distance metric is novel in
this work and differentiates it from \cite{Cussat-Blanc2015a}. This was found to
improve results in preliminary trials but is not presented as a part of this
study.

\subsection{Evolution}

Apart from the differences listed above, GRNEAT functions as a standard GA. The
mutation operations available during this work were
\begin{itemize}
  \item Modify (probability $p_{modify}=0.25$)
  \item Add a new regulatory protein with random parameters, $p_{add}=0.5$
  \item Delete $p_{delete}=0.25$
\end{itemize}
When mutating a genome, a random mutation operation was selected with
probability $p_{select}$. The delete mutation operation was not allowed when selected for
input and output genes.

During the crossover mutation, aligned proteins are randomly selected from
either parent with probability $p_{cross}=0.5$. If the parent genomes are of different
lengths, the unaligned regulatory proteins from the longer parent genome are
appended to the child genome with probability $p_{append}=0.5$.

